The Effects of Gravity on the Climate and Circulation of a Terrestrial Planet

The climate and circulation of a terrestrial planet are governed by, among other things, the distance to its host star, its size, rotation rate, obliquity, atmospheric composition and gravity. Here we explore the effects of the last of these, the Newtonian gravitational acceleration, on its atmosphere and climate. We first demonstrate that if the atmosphere obeys the hydrostatic primitive equations, which are a very good approximation for most terrestrial atmospheres, and if the radiative forcing is unaltered, changes in gravity have no effect at all on the circulation except for a vertical rescaling. That is to say, the effects of gravity may be completely scaled away and the circulation is unaltered. However, if the atmosphere contains a dilute condensible that is radiatively active, such as water or methane, then an increase in gravity will generally lead to a cooling of the planet because the total path length of the condensible will be reduced as gravity increases, leading to a reduction in the greenhouse effect. Furthermore, the specific humidity will decrease, leading to changes in the moist adiabatic lapse rate, in the equator-to-pole heat transport, and in the surface energy balance because of changes in the sensible and latent fluxes. These effects are all demonstrated both by theoretical arguments and by numerical simulations with moist and dry general circulation models.

==> preamble.tex <==
% -------------------------------------------------------------
% This file contains abbreviations, mainly mathematical
% -------------------------------------------------------------
%\sloppy
\RequirePackage{amsmath}
\RequirePackage{varioref}
\RequirePackage{myparalist}
\allowdisplaybreaks

\providecommand{\bmdefine}{}
\renewcommand{\bmdefine}[2]{\mycommand{#1}{{\bm{#2}}}}
\providecommand{\mathbfup}{\mathbf}


\newcounter{regequation}
\newcounter{mycounter}
\setcounter{secnumdepth}{2}

\newcommand{\newcm}[2]{\newcommand*{#1}{\ensuremath{#2}}}
\newcommand{\renewcm}[2]{\renewcommand*{#1}{\ensuremath{#2}}}
\newcommand{\newc}{\newcommand*}
\newcommand{\mycommand}[2]{\providecommand{#1}{} \renewcommand{#1}{#2}}

\renewcommand{\boxed}[1]{\fbox{$\displaystyle#1$}\,}

\providecommand{\what}{\widehat}
\providecommand{\wtilde}{\widetilde}

%\newcommand{\tablesection}[1]{\subsection*{\centering\large #1} \medskip }

% Need to redefine this because cupbook doesn't make the environment
% narrower, so the quotes are too wide. 
\renewenvironment{quote}
 {\begin{list}{}
 {%\setlength{\leftmargin}{1cm}
 \setlength{\rightmargin}{\leftmargin}}
 \item[]}%
  {\end{list}}
  

\newenvironment*{myquote}[2]{  \begin{quote}
 %{\small\textit{\textsf{#1}}} \\ \textsf{\footnotesize  #2}  } 
 {\small\itsf#1} \\ \textsf{\footnotesize  #2}  } 
{ \end{quote} }
 
\newenvironment*{chapquote}[2]{  \begin{savequote} 
  {\small\textit{\textsf{#1}}} \vskip 2pt  {\sf \footnotesize {#2}}  } 
{ \end{savequote} }

% \renewenvironment*{myquote}[2]{\begin{quote} \begin{flushright} 
% \textit{\textsf{\small  #1 } } \\ \textsf{\footnotesize  #2}  }
% { \end{flushright} \end{quote} }


\newenvironment{shtable}[1][tbp]
   {\begin{table}[#1]\begin{center}\begin{minipage}{\tablewidth}\begin{shaded}
   \begin{minipage}{\tablewidth}
   \setcounter{regequation}{\value{equation}}\setcounter{equation}{0}
   \renewcommand{\theequation}{\arabic{equation}}
   %\parskip=0pt 
   \parindent=0.5cm 
   \normalsize
   }%
  {\setcounter{equation}{\value{regequation}}
    \end{minipage}\end{shaded}\end{minipage}\end{center}\end{table} }

\newenvironment{wshtable}[1][tbp]
{\begin{table}[#1]\begin{center}\begin{minipage}{1.0\textwidth}\begin{shaded}
   \begin{minipage}{\textwidth}
    \setcounter{regequation}{\value{equation}}\setcounter{equation}{0}
   \renewcommand{\theequation}{\eqnbox.\arabic{equation}}
   %\parskip=0pt
   \parindent=0.5cm 
   \normalsize
   }%
  {\setcounter{equation}{\value{regequation}}
   \end{minipage}\end{shaded}\end{minipage}\end{center}\end{table} }

\newenvironment{frtable}[1][tbp]
   {\begin{table}[#1]\begin{center}\begin{boxedminipage}{\tablewidth}
   \setcounter{regequation}{\value{equation}}\setcounter{equation}{0}
   \renewcommand{\theequation}{\arabic{equation}}
    \parindent=0.5cm \normalsize}%
 {\setcounter{equation}{\value{regequation}}
   \end{boxedminipage}\end{center}\end{table} }
   
   \newenvironment{wfrtable}[1][tbp]
      {\begin{table}[#1]\begin{center}\begin{boxedminipage}{\textwidth}
      \setcounter{regequation}{\value{equation}}\setcounter{equation}{0}
      \renewcommand{\theequation}{\arabic{equation}}
       \parindent=0.5cm \normalsize}%
    {\setcounter{equation}{\value{regequation}}
      \end{boxedminipage}\end{center}\end{table} }


\newenvironment{notes}{ \begin{small} \begin{sffamily} 
\renewcommand{\rightmark}{Notes and Problems}
   \setlength{\rightmargin}{0.\leftmargin}}   % see also enoteformat in 
                                              % mysects.sty
   {\end{sffamily} \end{small}}


% This is the environment for the problem sets 
\newenvironment{problems}{\begin{sffamily} \begin{small} 
\renewcommand{\rightmark}{Notes and Problems}
 \setcounter{equation}{0}
 \renewcommand{\theequation}{P\thechapter.\arabic{equation}}
 \subsubsection*{Problems}
 \begin{list}{\thechapter.\arabic{mycounter}} 
   {\usecounter{mycounter}\setlength{\itemsep}{2pt}
%   \setlength{\leftmargin}{1cm}\setlength{\rightmargin}{1cm}}}%
   \setlength{\rightmargin}{0.\leftmargin}}}%                                                              
  {\newpage \end{list} \end{small} \end{sffamily} \renewcommand{\rightmark}{Problems} }
%   
  
  
% This is for the problem sets of chapter 1.
 \newenvironment{problemsch1}{\begin{sffamily} \begin{small}
 \renewcommand{\rightmark}{Notes and Problems}
 \setcounter{equation}{0}\renewcommand{\theequation}{P\thechapter.\arabic{equation}}
 \begin{list}{\thechapter.\arabic{mycounter}}
   {\usecounter{mycounter}\setlength{\itemsep}{2pt} 
 % \setlength{\leftmargin}{1cm}\setlength{\rightmargin}{1cm}}}%
   \setlength{\rightmargin}{0.\leftmargin}}}%
   {\newpage \end{list} \end{small} \end{sffamily}}
  

% \newcommand{\theenotes}{\begingroup
% 	\setlength{\parskip}{1ex}
% 	\renewcommand{\enoteheading}{\subsubsection*{Notes} 
% 		   \leavevmode\par\vskip-0.8\baselineskip }
% 	\renewcommand{\enotesize}{\small}
% 	\theendnotes \setcounter{endnote}{0} \endgroup}	

\newcommand{\theenotes}{\begingroup
        \setlength{\parskip}{1ex}
        \renewcommand{\enoteheading}{}
        \renewcommand{\enotesize}{\small}
        \bigskip \par \pagebreak[3] 
        \noindent {\normalsize \itsf Notes} \nopagebreak
        \theendnotes \setcounter{endnote}{0}  \endgroup}


%\def\enoteformat{\rightskip\z@ \leftskip 1cm \parindent=0em
%     \leavevmode\llap{\hbox{{\@theenmark.} }}}




\newenvironment{ndes}{ \begin{small} \begin{sffamily}
\begin{list}{}{\usecounter{mycounter}
\setlength{\itemindent}{-0.6cm} %
\setlength{\topskip}{0pt}
\setlength{\parsep}{0pt}
%\setlength{\leftmargin}{1cm} %\setlength{\rightmargin}{1cm}}}%
\setlength{\rightmargin}{0.\leftmargin}}}%
{\end{list}\end{sffamily}\end{small}}


\newenvironment{ndes3}{ 
\begin{compactdesc} 
    \setlength{\topskip}{-10pt}
\setlength{\itemindent}{-0.6cm} }
{\end{compactdesc}}

\newenvironment{ndes2}{ \begin{small} \begin{sffamily}
\begin{list}{}{\usecounter{mycounter}
\setlength{\itemindent}{-0.6cm} %
\setlength{\topskip}{0pt}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt} \setlength{\parskip}{-50pt} \setlength{\partopsep}{0pt} 
%\setlength{\leftmargin}{1cm} %\setlength{\rightmargin}{1cm}}}%
\setlength{\rightmargin}{0.\leftmargin}}}%
{\end{list}\end{sffamily}\end{small}}


\newenvironment{enumar}{\begin{list}{\arabic{mycounter}.}{\usecounter{mycounter}
\setlength{\rightmargin}{\leftmargin}}}%
 {\end{list}}

\newenvironment{enumi}{\begin{list}{(\roman{enumi})}{\usecounter{enumi}
\setlength{\rightmargin}{\leftmargin}}}%
 {\end{list}}

\newenvironment{enumI}{\begin{list}{\Roman{mycounter}}{\usecounter{mycounter}
\setlength{\rightmargin}{\leftmargin}}}%
 {\end{list}}

 \newenvironment{enumalph}{\begin{list}{(\alph{enumi})}{\usecounter{enumi}
 \setlength{\rightmargin}{0.\leftmargin}}}%
 {\end{list}}

\newenvironment*{equationab}{\begin{equation}\eqnab}{\end{equation}}
\newcommand{\eqnab}%
    {\renewcommand{\theequation}{\arabic{chapter}.\arabic{equation}a,b}}
\newcommand{\eqnabc}%
    {\renewcommand{\theequation}{\arabic{chapter}.\arabic{equation}a,b,c}}
	\newcommand{\eqnc}%
	    {\renewcommand{\theequation}{\arabic{chapter}.\arabic{equation}c}}
\newcommand{\eqnabbox}%
   {\renewcommand{\theequation}{\eqnbox.\arabic{equation}a,b}}
\newcommand{\eqnbox}{BOX}
\newcommand{\defeqnbox}[1]{\renewcommand{\eqnbox}{#1}}
    

\newcommand{\aleqnab}%
	{\renewcommand{\theequation}{\theparentequation{a,b}}}
	\newcommand{\aleqnbc}%
		{\renewcommand{\theequation}{\theparentequation{b,c}}}
	\newcommand{\aleqnc}%
	{\renewcommand{\theequation}{\theparentequation{c}}}
	\newcommand{\aleqnabc}%
		{\renewcommand{\theequation}{\theparentequation{a,b,c}}}
		\newcommand{\aleqna}%
		{\renewcommand{\theequation}{\theparentequation{a}}}

\newcommand{\textcas}{\texttt}
\newenvironment{casual}{\ttfamily\itshape}{}

\newcommand{\itref}[1]{{\itshape(\ref{#1})}}
\newcommand{\euro}{\textsf{\texteuro}}
\newcommand{\ppt}{\textperthousand \xspace}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\itsf}{\itshape\sffamily}
\newcommand{\textitsf}[1]{\textit{\textsf{#1}}}

\newcommand{\bindex}[1]{\index{#1|textbf} }
\newcommand{\secindex}[1]{\index{#1|(textbf} }
\newcommand{\esecindex}[1]{\index{#1|)textbf} }
\newcommand{\mybegindex}[1]{\index{#1|(} }
\newcommand{\myendindex}[1]{\index{#1|)} }

%\providecommand{\PARENS}[1]{\left( #1 \right)}
\newcommand{\bracket}[1]{\left( #1 \right)}
\newcommand{\sbracket}[1]{\left[ #1 \right]}
\newcommand{\cbracket}[1]{\left\{ #1 \right\} }
\newcommand{\abracket}[1]{\left\langle #1 \right\rangle}
\newcommand{\bracksup}[2]{\bracket{#1}^{\!\!#2}}
\newcommand{\bracksub}[2]{\bracket{#1}_{\!\!#2}}
\newcommand{\lbracksub}[2]{\left.{#1}\right|_{#2}}
\newcommand{\linesub}[1]{\left.\right|_{#1}}
\newcommand{\ave}[1]{\left< #1 \right> }
\newcommand*{\unit}[1]{\ensuremath{\mathrm{\,#1}}}

\providecommand{\bneg}{\mkern -3mu} % negative space for subscripts after large brackets.
\providecommand{\bnegsup}{\bneg} % negative space for superscripts after large brackets.

%\renewcommand{\bracket}{\PARENS}

%\def\gobble #1{}   % effectively comments out what is in curly brackets
\newcommand{\gobble}[1]{\!}
\renewcommand{\Re}{\text{Re}\,}
\newcommand{\Rey}{\mathit{Re}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\etascale}{\mathcal H}

\newc{\x}{$x$\xspace} \newc{\y}{$y$\xspace}  \newc{\z}{$z$\xspace}
\newcommand{\sgn}{\text{sgn}\xspace}

\newcommand{\APE}{\textit{APE}\xspace}
\newcommand{\KE}{\textit{KE}\xspace}
\newcommand{\PE}{\textit{PE}\xspace}
\newcommand{\TPE}{\textit{TPE}\xspace}
%\newc{\afterpag}{\afterpage}
\renewcommand{\O}{\ensuremath{\mathcal{O}}}
\newcommand{\obar}[2][]{\overline{#2}^{#1}}
\newcommand{\inprod}[2]{\left\langle{#1},{#2}\right\rangle}
\newc{\probref}[1]{\thechapter.\ref{#1}}
\providecommand{\LettrineFontHook}{}
\renewcommand{\LettrineFontHook}{\sffamily}
\newc{\letrn}[2]{\lettrine[lines=3,lhang=0]{{\color{gray}#1}}
               {\MakeUppercase{\footnotesize\sffamily #2}}}
	      % {#2}  } 
\newc{\figref}[1]{Fig.~\ref{#1}}
\newc{\Figref}[1]{Figure \ref{#1}}
\newc{\secref}[1]{Section \ref{#1}}
\newcommand{\enote}[1]{$^{\ref{#1}}$}
\newc{\dbint}{\iint}
\newcommand{\curl}{\nabla\cross}
\newc{\curlz}{\mathrm{curl}_z}
\renewcommand{\div}[1][]{\nabla_{\! #1} \cdot}
\newcommand{\divh}{\nabla_h \cdot}
\newcommand{\divm}{\nabla_m \cdot}
\newcommand{\dg}{\text{\textdegree}\xspace}
\newcommand{\dgc}{\text{\textdegree\,C}\xspace}
\newcommand{\dgs}{\text{\textdegree\,S}\xspace}
\newcommand{\dgn}{\text{\textdegree\,N}\xspace}
\newcommand{\dgw}{\text{\textdegree\,W}\xspace}
\newcommand{\dge}{\text{\textdegree\,E}\xspace}
%\newc{\dg}{\ensuremath{^\circ}\xspace}
\newcommand{\boxeq}[1]{\begin{equation}
      \fbox{$\displaystyle{#1}$} \end{equation}}
\newcommand{\myboxed}[1]{\ovalbox{$\displaystyle{#1}$}}
%\newcommand{\dsty}{\displaystyle}
\renewcommand{\sup}[1]{^{(#1)}}
\newcommand{\eqn}[1]{\( \displaystyle{#1} \)}
\bmdefine{\omb}{\omega}
\bmdefine{\Omb}{\varOmega}
\newcommand{\ombhat}{\widehat{\omb}}
\newcommand{\ombsw}{\omb^*}
\newcommand{\tvb}{\wtilde{\vb}}
\newcommand{\tub}{\wtilde{\ub}}
\providecommand{\ubtil}{\wtilde{\ub}}
\providecommand{\vbtil}{\wtilde{\vb}}
\mycommand{\wbtil}{\wtilde{\wb}}
\bmdefine{\taub}{\tau}
\bmdefine{\deltab}{\delta}
\newc{\ttaub}{\wtilde{\taub}}
\newc{\ttau}{\wtilde\tau}
\newcommand{\trho}{\wtilde \rho}
\newcommand{\ttheta}{\wtilde \theta}
\newcommand{\tsigma}{\wtilde \sigma}
\newcommand{\e}{\mspace{1mu} \mathrm{e}\mspace{1mu}}
\newcommand{\er}{\mspace{1mu} \mathrm{e}\mspace{1mu}}
\newcommand{\Er}{\mspace{1mu} \mathrm{E}\mspace{1mu}}
\newcommand{\ir}{\mathrm{i}\mspace{1mu}}
\newc{\s}{\,\text{s}\xspace} 
\mycommand{\m}{\,\text{m}\xspace}
\newc{\cm}{\,\text{cm}\xspace}
\newc{\km}{\,\text{km}\xspace}
\newc{\kg}{\,\text{kg}\xspace}
\newcm{\ps}{\,\text{s}{^{-1}}\xspace}
\newc{\mps}{\ensuremath{\m\ps}\xspace}
\newc{\Kv}{\,\text{K}\xspace}
\newc{\Sv}{\,\text{Sv}\xspace}
\newc{\hpa}{\,\text{hPa}\xspace}
\newc{\hPa}{\,\text{hPa}\xspace}
\newc{\rms}{\text{rms}}
\newc{\qg}{quasi-geostrophic\xspace}
\newc{\pg}{planetary-geostrophic\xspace}
\newc{\BV}{Brunt--V\"ais\"al\"a\xspace}
\newcommand{\elnino}{El Ni\~no\xspace}
\newc{\Elnino}{El NI\~NO\xspace}
\newc{\crn}{\nonumber  \\}
\newc{\qqquad}{\qquad \qquad}
\newc{\cdel}{\cdot \nabla}
\newcommand{\cg}{c_{g}}
\newcommand{\cgx}{c_{g}^x}
\newcommand{\cgy}{c_{g}^y}
\newcommand{\cgz}{c_{g}^z}
\newcommand{\cbg}{\bm{c}_{g}}
\newcommand{\cgb}{\bm{c}_{g}}
%\renewcommand{\div}[1][]{\nabla_{#1}\cdot}
\newcommand{\eten}[1]{\ensuremath{\times 10^{#1}}\xspace}
%\newc{\Ro}{\ensuremath{R_o}\xspace}
\newc{\Ro}{\ensuremath{\mathit{Ro}}\xspace}
\renewcommand{\Pr}{\ensuremath{\mathit{Pr}}\xspace}
\newc{\Ek}{\ensuremath{\mathit{Ek}}\xspace}
\newc{\Ra}{\ensuremath{\mathit{Ra}}\xspace}
\newc{\Fr}{\ensuremath{\mathit{Fr}}\xspace}
\newc{\Bu}{\ensuremath{\mathit{Bu}}\xspace}
\newc{\Ri}{\ensuremath{\mathit{Ri}}\xspace}
\newc{\Rot}{\ensuremath{\mathit{Ro_\mathrm{t}}}\xspace}
\newcommand{\ro}{\ensuremath{\rho_0} }
\newcommand{\ptwo}[2]{{\partial^2 #1 \over \partial #2^2}}
\newcommand{\ppabc}[3]{{\partial^2 #1 \over \partial #2 \partial #3 }}
\newcommand{\pptwo}[2]{{\partial^2 #1 / \partial #2^2}}
\newc{\bpp}[2]{\bfrac{\partial #1}{\partial #2}}
\newc{\bppp}[2]{({\partial #1}/{\partial #2})}
\newc{\bfrac}[2]{\left( \frac{#1}{#2} \right) }
\newc{\textfrac}[2]{{(#1)}/{(#2)}}
\newc{\dbfrac}[2]{\left( \dfrac{#1}{#2} \right) }
\newc{\bfracs}[3]{\left(\frac{#1}{#2}\right)_{\bneg #3}}
\newc{\bfracsub}[3]{\left(\frac{#1}{#2}\right)_{\bneg #3}}
\newc{\bfracsup}[3]{\left(\frac{#1}{#2}\right)^{\bnegsup #3}}
\newc{\bpps}[3]{\left(\frac{\partial #1}{\partial #2}\right)_{\bneg #3}}
\newc{\bppsub}[3]{\left(\frac{\partial #1}{\partial #2}\right)_{\bneg #3}}
\newc{\bppsup}[3]{\left(\frac{\partial #1}{\partial #2}\right)^{\bnegsup #3}}
\newc{\bdds}[3]{\left(\frac{\d #1}{\d #2}\right)_{\bneg #3}}
\newcommand{\bracsup}[2]{\bracket{#1}^{\bnegsup #2} }
\newcommand{\bracsub}[2]{\bracket{#1}_{\bneg #2} }
\newcommand{\qtext}[1]{\quad \text{#1} \quad} 
\newcommand{\qqtext}[1]{\qquad \text{#1} \qquad}

\mycommand{\T}{\mathcal{T}}
\mycommand{\C}{\mathcal{C}}
\mycommand{\Eta}{\mathcal{E}}
\mycommand{\Zeta}{\mathcal{Z}}
\newcommand{\Peta}{\mathcal{P}}
\newc{\K}{\mathcal{K}}
\newcommand{\bta}{\ensuremath{\beta}\xspace}
\newcommand{\ustar}{\ensuremath{{u^*}} }
\newc{\psisp}[1]{\psi^{(#1)}}
\newcommand{\psidag}{\psi^\dagger}
\newc{\psibar}{\overline \psi}
\newc{\Psibar}{\overline \Psi}
\newc{\phibar}{\overline \phi}
\newc{\thetabar}{\overline \theta}
\newc{\varthetabar}{\overline \vartheta}
\newc{\varphibar}{\overline \varphi}
\renewcommand{\hbar}{\overline h}
\newcommand{\hbarr}{\overline h}
%\providecommand{\dtbar}{{\raisebox{2pt}{\mathchar'26}\mkern-12mu \d}} 
\newcommand{\mydbar}{~{\raisebox{0.85ex}{\smaller[2]--}\mkern-11.5mu \d \mkern 1mu}} 
\newcommand{\smalldbar}{~{\raisebox{0.6ex}{\smaller[4]--}\mkern-11.5mu \d \mkern 1mu}} 
\newc{\qbar}{\overline q}
\newc{\ubar}{\overline u}
\newc{\vbar}{\overline v}
\newcommand{\mbar}{\overline m}
\providecommand{\wbar}{}
\renewcommand{\wbar}{\overline w}
\newc{\ubbar}{\overline \ub}
\newc{\vbbar}{\overline \vb}
\newc{\bbar}{\overline b}
\newc{\pbar}{\overline p}
\newc{\zbar}{\overline z}
\newc{\rhobar}{\overline \rho}
\newc{\Fbar}{\overline F}
\newc{\Jbar}{\overline J}
\newc{\Sbar}{\overline S}
\newc{\Tbar}{\overline T}
\newc{\bybar}{\overline \by}
\newcommand{\sigmabar}{\overline \sigma}
\newc{\zetabar}{\overline \zeta}
\newc{\etabar}{\overline \eta}
\newc{\betahat}{\ensuremath{\what \beta}}
\newc{\kbeta}{k_\beta}
\newc{\that}{{\what t}}
\newc{\khat}{{\what k}}
\newcommand{\phat}{\what p}
\providecommand{\zetahat}{\ensuremath{\what \zeta}}
\newc{\deltahat}{\what \delta}
\newc{\etahat}{\what \eta}
\newc{\ubhat}{\what\ub}
\newc{\vbhat}{\what\vb}
\newc{\xhat}{{\what x}}
\newc{\xbhat}{{\what \xb}}
\newc{\yhat}{{\what y}}
\newc{\zhat}{{\what z}}
\newc{\uhat}{\what u}
\newc{\vhat}{\what v}
\newcommand{\Fhat}{\what F}
\newcommand{\chat}{\what c}
\providecommand{\hatw}{\what w}
\newc{\bhat}{\what b}
\newc{\fbhat}{\what{\bm{f}}}
\newc{\phihat}{\what \phi}
\newc{\byhat}{\what \by}
\newc{\hhat}{\ensuremath{\what h}}
\newc{\fhat}{\ensuremath{\what f}}
\newc{\psihat}{\what \psi}
\newc{\Psihat}{\what \Psi}
\newc{\Nhat}{\what N}
\newc{\Nbar}{\overline N}
\providecommand{\omegahat}{\what \omega}
\newc{\qhat}{\what q}

\newcommand{\weta}{\widetilde \eta}
\bmdefine{\jbi}{j}
\newcommand{\KEbar}{\overline{\KE}} 
\newcommand{\PEbar}{\overline{\PE}}
\providecommand{\Atilde}{\wtilde{A}}
\newcommand{\Ftilde}{\wtilde{F}}
\newcommand{\shalf}{\tfrac 12}
\newcommand{\lhat}{\widehat l}
\providecommand{\mhat}{\what m}
\newcommand{\fohat}{\what \fo}
\newcommand{\delhat}{\what \nabla}
\newcommand{\divhat}{\what \nabla \cdot}
\newcommand{\psitil}{\wtilde \psi}
\newcommand{\psitilde}{\psitil}
\newcommand{\phitil}{\wtilde \phi}
\newcommand{\htilde}{\wtilde h}
\newcommand{\tautil}{\wtilde \tau}
\newcommand{\zetatil}{\wtilde \zeta}
\newcommand{\etatil}{\wtilde \eta}
\newcommand{\htil}{\wtilde h}
\newcommand{\lint}{\mathlarger{\int}}

% \newfont{\lucid}{hlhr8r at 9pt}
% \newfont{\lucidl}{hlhr8r at 10pt}
% \renewcommand{\texttilde}{\lucid \textasciitilde}
% \newcommand{\texttildel}{\lucidl \textasciitilde}

\DeclareMathSymbol{\mywidetilde}{\mathord}{largesymbols}{"65}
\DeclareMathSymbol{\mywidehat}{\mathord}{largesymbols}{"62}
\renewcommand{\hatw}{ \mkern 5mu {\mywidehat \mkern-14mu w \mkern 1mu}}
\renewcommand{\mhat}{ \mkern 5mu {\mywidehat \mkern-14mu m \mkern 1mu}}
%\newcommand{\myhat}[1]{\mkern 3mu {\mywidehat \mkern-12mu #1 \mkern 1mu}}
%\newcommand{\mytilde}[1]{\mkern 3mu {\mywidetilde \mkern-12mu #1 \mkern 1mu}}

\newcommand{\util}{\mkern 2mu {\mywidetilde \mkern-12mu u \mkern 0mu}}
\newcommand{\vtil}{\mkern 2mu {\mywidetilde \mkern-12mu v \mkern 0mu}}
\providecommand{\wtil}{\mkern 4mu {\mywidetilde \mkern-14mu w \mkern 0mu}}
\providecommand{\Wtil}{\mkern 5mu {\raisebox{2pt}{$\mywidetilde$} \mkern-15mu W \mkern 1mu}}
\renewcommand{\omegahat}{\mkern 4mu {\mywidehat \mkern-14mu \omega \mkern 0mu}}

% use the following if mathtimes fonts are used
 % \renewcommand{\util}{\wtilde u}
 % \renewcommand{\vtil}{\wtilde v}
 % \renewcommand{\wtil}{\wtilde w}
 % \renewcommand{\omegahat}{\what \omega}
 % \renewcommand{\mhat}{\what m}

\newcommand{\Wtilde}{\Wtil}
\newcommand{\vtilde}{\vtil}
\newcommand{\utilde}{\util}
\providecommand{\wtill}{\wtil}
\providecommand{\tildew}{\wtil}

\renewcommand{\ubtil}{\mkern 2mu {\mywidetilde \mkern-12mu \ub \mkern 0mu}}
\renewcommand{\vbtil}{\mkern 2mu {\mywidetilde \mkern-12mu \vb \mkern 0mu}}
\renewcommand{\wbtil}{\mkern 4mu {\mywidetilde \mkern-14mu \wb \mkern 0mu}}

\newcommand{\phitilde}{\wtilde \phi}
\providecommand{\Phitilde}{\wtilde \Phi}
\newcommand{\Phihat}{\what \Phi}
\newcommand{\ptil}{\wtilde p} \newcommand{\ptilde}{\wtilde p}
\newc{\tauhat}{\what \tau}
\newcommand{\Ehat}{\what E}
\newcommand{\Zhat}{\what Z}
\mycommand{\Ebar}{\overline E}
\mycommand{\Zbar}{\overline Z}
\newcommand{\rhs}{right-hand side\xspace}
\newc{\ug}{u_g}
\newc{\vg}{\ensuremath{v_g}\xspace}
\newc{\Lr}{\Ld}
\newcommand{\Ld}{\ensuremath{L_{d}}\xspace}
\newcommand{\kd}{\ensuremath{k_{d}}\xspace}
\newc{\lr}{\ensuremath{l_r}}
\newc{\lrr}{\ensuremath{\lambda_r}}
\newc{\vrt}{\vartheta}
%\newc{\cross}{\bm{\times}}
\newc{\cross}{\times}
%\newc{\half}{\tfrac 12}
\newc{\half}{\frac 12}
\newc{\third}{\frac 13}
\newc{\quarter}{\frac 14}
\def\dF{\, \mathrm{d} \bm{F}}
\def\dl{\, \mathrm{d}{l}}
\def\dlb{\, \mathrm{d} \bm{l}}
\def\drb{\mathrm{d} \bm{r}}
\def\dV{\, \mathrm{d}V}
\newc{\dt}{\, \mathrm{d}t}
\newc{\dx}{\, \mathrm{d}x}
\newc{\dy}{\, \mathrm{d}y}
\mycommand{\dz}{\, \mathrm{d}z}
\newc{\dk}{\, \mathrm{d}k}
\newc{\dr}{\, \mathrm{d}r}
\newc{\dkb}{\, \mathrm{d}\bm{k}}
\newc{\dxb}{\, \mathrm{d}\xb}
\newc{\dvrt}{\, \mathrm{d}\vrt}
\newc{\dpr}{\, \mathrm{d}p}
\newcommand{\dtheta}{\, \mathrm{d}\theta}
\def\dS{\, \mathrm{d} S}
\def\dSb{\, \mathrm{d} \bm{S}}
\def\dA{\, \mathrm{d}{A}}
\newc{\dAb}{\, \mathrm{d} \bm{A}}
\newc{\Dth}{{\D_h \over \D t}}
\newc{\Dto}{{\D_0 \over \D \that}}
\newc{\Fb}{\bm{F} }
\bmdefine\Fb{F}
\newcommand{\Mb}{\bm{M} }
\newcommand{\Sb}{\ensuremath{\bm{S}}\xspace}
\newc\Ab{\ensuremath{\bm{A}}}
\newc\Cb{\ensuremath{\bm{C}}}
\newc\Jb{\ensuremath{\bm{J}}}
\newc\Bb{\ensuremath{\bm{B}}}
\newc\xb{{\bm{x}}}
\bmdefine{\pb}{p}
\bmdefine{\qb}{q}
\bmdefine{\ab}{a}
\bmdefine{\Xb}{X}
\bmdefine{\Yb}{Y}
\bmdefine{\rb}{r}
\newcommand{\rbb}{\mathbf{r}}
%\renewcommand*{\sb}{\bm{s}}
\bmdefine{\sb}{s}
\bmdefine{\Db}{D}
\def\bb{{\ensuremath{\bm {b}}}}
\def\gb{\bm{g} }
\newcommand\ib{\mathbf{i}}
\newcommand\jb{\mathbf{j}}
\newcommand{\kb}{{\bf k}}
\bmdefine{\kbi}{k}
\bmdefine{\jbi}{j}
\bmdefine{\Vb}{V}
\bmdefine{\Wb}{W}
\def\lb{{\bm l} }
\newc{\fb}{{\ensuremath{\bm {f}}}}
\newc{\fbo}{{\ensuremath{\bm {f}_0}}}
\def\vb{{\ensuremath{\bm {v}}}\xspace}
\def\ub{{\ensuremath{\bm {u}}}\xspace}
\def\wb{{\ensuremath{\bm {w}}}\xspace}
\def\mb{{\ensuremath{\bm {m}}}\xspace}
\def\nb{{\ensuremath{\bm {n}}}\xspace}
\bmdefine{\Ub}{U}
\bmdefine{\cb}{c}
\bmdefine{\psib}{\psi}
\bmdefine{\phib}{\phi}
\def\dll{\delta \lb}
\def\dlrb{\delta \rb}

\newcommand{\by}{\ensuremath{b}}

\newc{\Tb}{{\bm T} }
\newc{\lhs}{left-hands side\xspace}
\newc{\fo}{\ensuremath{f_0}\xspace}
\def\DD#1{{\D#1 \over \D t}}
\newcommand{\DDhat}[1]{{\D#1 \over \D \that }}
\newcommand{\DDDhat}[1]{{\D#1 / \D \that }}
\newcommand{\DDbar}[1]{{\overline{\D}#1 \over \D t}}
\def\DDh#1{{\D_h#1 \over \D t}}
\def\DDo#1{{\D_0#1 \over \D \that}}
\newc{\MD}[1]{{\partial {#1} \over \partial t} + (\vb \cdot \del) #1}
\def\Dt{{\D \over \D t}} 
\newcommand{\pp}[3][]{\frac{\partial^{#1} #2}{\partial #3^{#1}}}
\newcommand{\ppp}[3][]{{\partial^{#1} #2 / \partial #3^{#1}}}
\newcommand{\pppp}[3][]{{\partial^{#1}_{#3} #2 }} 
\newcommand{\DDD}[1]{\D{#1} / \D t}
\newcommand{\ddd}[3][]{{\d^{#1} #2 / \d #3^{#1}}}
\newc{\ppa}[1]{{\partial \over \partial #1}}
\newc{\pt}{{\partial \over \partial t}}
\newc{\dell}[1][]{\nabla_{\!#1\,}}
\newc{\del}{\nabla}
\newc{\grad}{\nabla}
\newc{\delh}{\nabla_h}
\newc{\cp}{c_{p}}
\newc{\cv}{c_{v}}
\def\kv{\kappa_v}
\def\kh{\kappa_h}
\newcommand{\kvy}{\kappa^\mathit{vy}}
\newcommand{\kvz}{\kappa^\mathit{vz}}
\newcommand{\kwy}{\kappa^\mathit{wy}}
\newcommand{\kwz}{\kappa^\mathit{wz}}
\newcommand{\srho}{s_{\rho}}
\newcommand{\Kt}{\ensuremath{\tensor{K}}\xspace}
\newcommand{\St}{\ensuremath{\tensor{S}}\xspace}
\newcommand{\At}{\ensuremath{\tensor{A}}\xspace}
\newcommand*{\veps}{\varepsilon}
\newcommand*{\eps}{\epsilon}
\def\delsq{\nabla^2}
\newcommand{\delsqhat}{\what\del^2}
\newcommand{\Jhat}{\what J}
\def\delsqh{\nabla^2_h}
\def\delt{\nabla^2}
\def\delth{\nabla^2_h}
\newcommand{\dd}[3][]{{\d^{#1} #2 \over \d #3^{#1}}}
\newcommand{\dif}{\mathrm{d}}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\f}{$f$\xspace}
\newcommand{\D}{\mathrm{D}}
%\newcommand{\vres}[1][]{\obar{v^*_{#1}}}
\newcommand{\vres}[1][]{\overline v_{\! #1}^{*}}
\renewcommand{\vres}[1][]{\ensuremath{\overline v_{\! #1}^{*}}\xspace}
\newcommand{\psires}{\psi^*}
\newcommand{\vbres}[1][]{\overline \vb_{\! #1}^{*}}
\newcommand{\ubres}[1][]{\overline \ub_{\! #1}^{*}}
\newcommand{\wres}[1][]{\overline w_{\! #1}^{*}}
%\newcommand{\Fbres}[1][]{\Fb_{#1}^{*}}
\newcommand{\Fbres}{\Fb^{*}}
\providecommand{\pref}{}
\renewcommand{\pref}{p_{R}}
\newcommand{\rhoref}{\rho_{R}} \newcommand{\rhor}{\rho_{R}}
\newcommand{\EN}{El Ni\~no\xspace}

%\newcommand{\eqref}[1]{\textup{\tagform@{\ref{#1}}}} % amsmath def
%\renewcommand{\eqref}[1]{(\ref{#1})} % gets fonts better than standard
\newcommand{\Eqref}[1]{Eq.\ (\ref{#1})} 
\newcommand{\eq}{\textit{eq}}  

\newcommand{\textmonth}{\ifcase\month \or January \or February\or
March\or April\or May \or June \or July\or August\or September\or October
\or November\or December\fi\xspace}

% Following line always works but is a cheap hack using text fonts in math.
\providecommand{\tensor}[1]{\textit{\textsf{\textbf{#1}}}}

% Following lines are better but may cause TeX to run out of math alphabets.
%\DeclareMathAlphabet{\mathsfsl}{\encodingdefault}{cmss}{bx}{sl} % uses cmr fonts
\DeclareMathAlphabet{\mathsfsl}{\encodingdefault}{hlst}{b}{sl}   % uses lucida
\renewcommand{\tensor}[1]{\mathsfsl{#1}}      % this is the delicate command
                                               % Leave it in if possible


\newcommand\longpage[1][1]{\enlargethispage{#1\baselineskip}}
\newcommand\shortpage[1][1]{\enlargethispage{-#1\baselineskip}}

\providecommand{\bibname}{}
\renewcommand{\bibname}{References}

\newc{\putabcd}{\put(-9.2,7){\small \textit{\textsf{(a)}}}
\put(-4.5,7){\small \textit{\textsf{(b)}}}
\put(-9.2,3.3){\small \textit{\textsf{(c)}}}
\put(-4.5,3.3){\small \textit{\textsf{(d)}}}
}

\newc{\putab}{\put(-8.9,3.3){\small \textit{\textsf{(a)}}}
\put(-4.3,3.3){\small \textit{\textsf{(b)}}}
}
\newcommand{\itemm}{\item\mbox{}}
%\newcommand{\topfigrule}{\vspace*{-3pt}
  %              \rule{\columnwidth}{0.4pt}\vspace{2.6pt} }
% ---------------------------------------------------------------
 
% Following lines ensure uniformity of mathcal between fontsets. 

%\DeclareMathAlphabet{\mathcal}  {OMS}{hlcy}{m}{n}  % uses lucida
%\SetMathAlphabet{\mathcal}{bold}{OMS}{hlcy}{b}{n}  % uses lucida for bold
%\DeclareMathAlphabet{\mathbcal} {OMS}{hlcy}{b}{n}  % don't need this


% \DeclareMathAlphabet{\mathcal}       {U}{mtms}{m}{n}
% \SetMathAlphabet    {\mathcal} {bold}{U}{mtms}{b}{n}

%Let's use cmr, for simplicity and style
%\DeclareMathAlphabet{\mathcal}  {OMS}{cmsy}{m}{n}
%\SetMathAlphabet{\mathcal}{bold}{OMS}{cmsy}{b}{n}
%%\DeclareMathAlphabet{\mathbcal} {OMS}{cmsy}{b}{n} % don't need this
                                                                                                  
\newcommand{\Fbc}{\bm{\mathcal F}}
\newcommand{\Fc}{\mathcal F}
\newcommand{\Gcal}{\mathcal G}


%\bmdefine{\Fbc}{\mathcal F}
\bmdefine{\Ebc}{\mathcal E}
%%\renewcommand{\Fbc}{\pmb{\mathcal{F}}} % comment out this line if possible
                                        % however, it may lead to too many
                                        % math alphabets (esp with mathtime)
                         
\newcommand{\resetcaptionmargin}{\setcaptionmargin{\captmarg}}
\newcommand{\iteml}[1]{\item\label{#1}}
\newcommand{\bfig}{\begin{figure}}
\newcommand{\efig}{\end{figure}}
\newcommand{\bcen}{\begin{center}}
\newcommand{\ecen}{\end{center}}
%\newcommand{\beql}[1]{\begin{equation}\label{#1}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}


\newcommand{\bsub}{\begin{subequations}}
\newcommand{\esub}{\end{subequations}}

%\renewcommand{\diamondsuit}{\blacklozenge}
% \renewcommand{\Omega}{\varOmega}
% \renewcommand{\Gamma}{\varGamma}
% \renewcommand{\Pi}{\varPi}

\renewcommand{\reftextcurrent}{above}
\newcommand{\eqvref}[1]{\eqref{#1}\ \vpageref{#1}}

% \DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
% \DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
% \DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}
% \providecommand{\vardiamondsuit}{\vardiamond}
% \providecommand{\diamondsuit}{}
% \AtBeginDocument{\renewcommand{\diamondsuit}{{^\vardiamondsuit}}}


\providecommand{\blacklozenge}{\vardiamondsuit}
\providecommand{\diamondsuit}{}
\AtBeginDocument{\renewcommand{\diamondsuit}{^{\blacklozenge}}}

